Taxonomy and Evaluation of Structured Compression of Convolutional Neural Networks

The success of deep neural networks in many real-world applications is leading to new challenges in building more efficient architectures. One effective way of making networks more efficient is neural network compression. We provide an overview of existing neural network compression methods that can be used to make neural networks more efficient by changing the architecture of the network. First, we introduce a new way to categorize all published compression methods, based on the amount of data and compute needed to make the methods work in practice. These are three 'levels of compression solutions'. Second, we provide a taxonomy of tensor factorization based and probabilistic compression methods. Finally, we perform an extensive evaluation of different compression techniques from the literature for models trained on ImageNet. We show that SVD and probabilistic compression or pruning methods are complementary and give the best results of all the considered methods. We also provide practical ways to combine them.

==> jmle2e_jmlr.tex <==
%
% File:    Macros for Journal of Machine Learning Research
%      Very minor modification of macros for Journal of Artificial 
%      Intelligence Research (jair.sty) 
%   Last edited October 9, 2000 by Leslie Pack Kaelbling
%   Last edited January 23, 2001 by Alex J. Smola (we should set up RCS or CVS)
%   Last edited March 29, 2004 Erik G. Learned-Miller
%   Last edited January 17, 2016 Charles Sutton 
%    (We have now set up GIT, good thing that we waited for it to
%     be invented.)
%
%          The name of this file should follow the article document
%          type, e.g. \documentstyle[jmlr]{article}

%          Copied and edited from similar file for Machine Learning Journal.
% Original Author:  Jeff Schlimmer
% Edited by: Kevin Thompson, Martha Del Alto, Helen Stewart, Steve Minton \& Pandu Nayak.
% Last edited: Mon  May  3 20:40:00 1993 by kthompso (Kevin Thompson) on muir

\typeout{Document Style `jmlr' -- January 2016.}

\newif\if@abbrvbib\@abbrvbibfalse
\DeclareOption{abbrvbib}{\@abbrvbibtrue}

\newif\if@usehyper\@usehypertrue
\DeclareOption{nohyperref}{\@usehyperfalse}
\DeclareOption{hyperref}{\@usehypertrue}

\DeclareOption*{\PackageWarning{jmlr}{Unknown ‘\CurrentOption’}}
\ProcessOptions\relax

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             REQUIRED PACKAGES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\RequirePackage{epsfig}
\RequirePackage{amssymb}
\RequirePackage{natbib}
\RequirePackage{graphicx}

\if@usehyper
\RequirePackage[colorlinks=false,allbordercolors={1 1 1}]{hyperref}
\fi

\if@abbrvbib
\bibliographystyle{abbrvnat}
\else
\bibliographystyle{plainnat}
\fi

\bibpunct{(}{)}{;}{a}{,}{,}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             P A G E   S I Z E
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
% Change the overall width of the page.  If these parameters are
%       changed, they will require corresponding changes in the
%       maketitle section.
%
\renewcommand{\topfraction}{0.95}   % let figure take up nearly whole page
\renewcommand{\textfraction}{0.05}  % let figure take up nearly whole page

% Specify the dimensions of each page

\oddsidemargin .25in    %   Note \oddsidemargin = \evensidemargin
\evensidemargin .25in
\marginparwidth 0.07 true in
%\marginparwidth 0.75 true in
%\topmargin 0 true pt           % Nominal distance from top of page to top of
%\topmargin 0.125in
\topmargin -0.5in
\addtolength{\headsep}{0.25in}
\textheight 8.5 true in       % Height of text (including footnotes & figures)
\textwidth 6.0 true in        % Width of text line.
\widowpenalty=10000
\clubpenalty=10000
\@twosidetrue \@mparswitchtrue \def\ds@draft{\overfullrule 5pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               S E C T I O N S
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Definitions for nicer (?) sections, etc., ideas from Pat Langley.
% Numbering for sections, etc. is taken care of automatically.

\def\@startsiction#1#2#3#4#5#6{\if@noskipsec \leavevmode \fi
   \par \@tempskipa #4\relax
   \@afterindenttrue
   \ifdim \@tempskipa <\z@ \@tempskipa -\@tempskipa \@afterindentfalse\fi
   \if@nobreak \everypar{}\else
     \addpenalty{\@secpenalty}\addvspace{\@tempskipa}\fi \@ifstar
     {\@ssect{#3}{#4}{#5}{#6}}{\@dblarg{\@sict{#1}{#2}{#3}{#4}{#5}{#6}}}}

\def\@sict#1#2#3#4#5#6[#7]#8{\ifnum #2>\c@secnumdepth
     \def\@svsec{}\else
     \refstepcounter{#1}\edef\@svsec{\csname the#1\endcsname}\fi
     \@tempskipa #5\relax
      \ifdim \@tempskipa>\z@
        \begingroup #6\relax
          \@hangfrom{\hskip #3\relax\@svsec.\hskip 0.1em}
                    {\interlinepenalty \@M #8\par}
        \endgroup
       \csname #1mark\endcsname{#7}\addcontentsline
         {toc}{#1}{\ifnum #2>\c@secnumdepth \else
                      \protect\numberline{\csname the#1\endcsname}\fi
                    #7}\else
        \def\@svsechd{#6\hskip #3\@svsec #8\csname #1mark\endcsname
                      {#7}\addcontentsline
                           {toc}{#1}{\ifnum #2>\c@secnumdepth \else
                             \protect\numberline{\csname the#1\endcsname}\fi
                       #7}}\fi
     \@xsect{#5}}

\def\@sect#1#2#3#4#5#6[#7]#8{\ifnum #2>\c@secnumdepth
     \def\@svsec{}\else 
     \refstepcounter{#1}\edef\@svsec{\csname the#1\endcsname\hskip 0.5em }\fi
     \@tempskipa #5\relax
      \ifdim \@tempskipa>\z@ 
        \begingroup #6\relax
          \@hangfrom{\hskip #3\relax\@svsec}{\interlinepenalty \@M #8\par}
        \endgroup
       \csname #1mark\endcsname{#7}\addcontentsline
         {toc}{#1}{\ifnum #2>\c@secnumdepth \else
                      \protect\numberline{\csname the#1\endcsname}\fi
                    #7}\else
        \def\@svsechd{#6\hskip #3\@svsec #8\csname #1mark\endcsname
                      {#7}\addcontentsline
                           {toc}{#1}{\ifnum #2>\c@secnumdepth \else
                             \protect\numberline{\csname the#1\endcsname}\fi
                       #7}}\fi
     \@xsect{#5}}

\def\thesection {\arabic{section}}
\def\thesubsection {\thesection.\arabic{subsection}}
\def\section{\@startsiction{section}{1}{\z@}{-0.24in}{0.10in}
             {\large\bf\raggedright}}
\def\subsection{\@startsection{subsection}{2}{\z@}{-0.20in}{0.08in}
                {\normalsize\bf\raggedright}}
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-0.18in}{0.08in}
                {\normalsize\sc\raggedright}}
\def\paragraph{\@startsiction{paragraph}{4}{\z@}{1.5ex plus
  0.5ex minus .2ex}{-1em}{\normalsize\bf}}
\def\subparagraph{\@startsiction{subparagraph}{5}{\z@}{1.5ex plus
  0.5ex minus .2ex}{-1em}{\normalsize\bf}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                              F O O T N O T E S
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Change the size of the footnote rule
%
% \renewcommand{\footnoterule}{\vspace{10pt}\hrule width 0mm}

\long\def\@makefntext#1{\@setpar{\@@par\@tempdima \hsize 
             \advance\@tempdima-15pt\parshape \@ne 15pt \@tempdima}\par
             \parindent 2em\noindent \hbox to \z@{\hss{\@thefnmark}. \hfil}#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               A B S T R A C T
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% use \begin{abstract} .. \end{abstract} for abstracts.
\renewenvironment{abstract}
{\centerline{\large\bf Abstract}\vspace{0.7ex}%
  \bgroup\leftskip 20pt\rightskip 20pt\small\noindent\ignorespaces}%
{\par\egroup\vskip 0.25ex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               KEYWORDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% use \begin{keywords} .. \end{keywords} for keywordss.
\newenvironment{keywords}
{\bgroup\leftskip 20pt\rightskip 20pt \small\noindent{\bf Keywords:} }%
{\par\egroup\vskip 0.25ex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                        FIRST PAGE, TITLE, AUTHOR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Author information can be set in various styles:
% For several authors from the same institution:
% \author{Author 1 \and ... \and Author n \\
%         \addr{Address line} \\ ... \\ \addr{Address line}}
% if the names do not fit well on one line use
%         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% To start a seperate ``row'' of authors use \AND, as in
% \author{Author 1 \\ \addr{Address line} \\  ... \\ \addr{Address line}
%         \AND
%         Author 2 \\ \addr{Address line} \\ ... \\ \addr{Address line} \And
%         Author 3 \\ \addr{Address line} \\ ... \\ \addr{Address line}}

% Title stuff, borrowed in part from aaai92.sty

\newlength\aftertitskip     \newlength\beforetitskip
\newlength\interauthorskip  \newlength\aftermaketitskip

%% Changeable parameters.
\setlength\aftertitskip{0.1in plus 0.2in minus 0.2in}
\setlength\beforetitskip{0.05in plus 0.08in minus 0.08in}
\setlength\interauthorskip{0.08in plus 0.1in minus 0.1in}
\setlength\aftermaketitskip{0.3in plus 0.1in minus 0.1in}

%% overall definition of maketitle, @maketitle does the real work
\def\maketitle{\par
 \begingroup
   \def\thefootnote{\fnsymbol{footnote}}
   \def\@makefnmark{\hbox to 0pt{$^{\@thefnmark}$\hss}}
   \@maketitle \@thanks
 \endgroup
\setcounter{footnote}{0}
 \let\maketitle\relax \let\@maketitle\relax
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}

\def\@startauthor{\noindent \normalsize\bf}
\def\@endauthor{}
\def\@starteditor{\noindent \small {\bf Editor:~}}
\def\@endeditor{\normalsize}
\def\@maketitle{\vbox{\hsize\textwidth
 \linewidth\hsize \vskip \beforetitskip
 {\begin{center} \Large\bf \@title \par \end{center}} \vskip \aftertitskip
 {\def\and{\unskip\enspace{\rm and}\enspace}%
  \def\addr{\small\it}%
  \def\email{\hfill\small\sc}%
  \def\name{\normalsize\bf}%
  \def\AND{\@endauthor\rm\hss \vskip \interauthorskip \@startauthor}
  \@startauthor \@author \@endauthor}

  \vskip \aftermaketitskip
  \noindent \@starteditor \@editor \@endeditor
  \vskip \aftermaketitskip
}}

\def\editor#1{\gdef\@editor{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% Pagestyle
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Defines the pagestyle for the title page.
%% Usage: \jmlrheading{1}{1993}{1-15}{8/93;}{9/93}
%%                      {Jane Q. Public and A. U. Thor}
%%        \jmlrheading{vol}{year}{pages}{Submitted}{published}{authors}

\def\firstpageno#1{\setcounter{page}{#1}}

\def\jmlrheading#1#2#3#4#5#6{\def\ps@jmlrtps{\let\@mkboth\@gobbletwo%
\def\@oddhead{\scriptsize Journal of Machine Learning Research #1 (#2) #3 \hfill Submitted #4; Published #5}%
\def\@oddfoot{\scriptsize \copyright #2 #6. \hfill}%
\def\@evenhead{}\def\@evenfoot{}}%
\thispagestyle{jmlrtps}}

%% Defines the pagestyle for the rest of the pages
%% Usage: \ShortHeadings{Minimizing Conflicts}{Minton et al}
%%        \ShortHeadings{short title}{short authors}

\def\ShortHeadings#1#2{\def\ps@jmlrps{\let\@mkboth\@gobbletwo%
\def\@oddhead{\hfill {\small\sc #1} \hfill}%
\def\@oddfoot{\hfill \small\rm \thepage \hfill}%
\def\@evenhead{\hfill {\small\sc #2} \hfill}%
\def\@evenfoot{\hfill \small\rm \thepage \hfill}}%
\pagestyle{jmlrps}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               MISCELLANY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Define macros for figure captions and table titles

% Figurecaption prints the caption title flush left.
% \def\figurecaption#1#2{\noindent\hangindent 42pt
%                        \hbox to 36pt {\sl #1 \hfil}
%                        \ignorespaces #2}
% \def\figurecaption#1#2{\noindent\hangindent 46pt
%                        \hbox to 41pt {\small\sl #1 \hfil}
%                        \ignorespaces {\small #2}}
\def\figurecaption#1#2{\noindent\hangindent 40pt
                       \hbox to 36pt {\small\sl #1 \hfil}
                       \ignorespaces {\small #2}}
% Figurecenter prints the caption title centered.
\def\figurecenter#1#2{\centerline{{\sl #1} #2}}
\def\figurecenter#1#2{\centerline{{\small\sl #1} {\small #2}}}

%
%  Allow ``hanging indents'' in long captions
%
\long\def\@makecaption#1#2{
   \vskip 10pt 
   \setbox\@tempboxa\hbox{#1: #2}
   \ifdim \wd\@tempboxa >\hsize               % IF longer than one line:
       \begin{list}{#1:}{
       \settowidth{\labelwidth}{#1:}
       \setlength{\leftmargin}{\labelwidth}
       \addtolength{\leftmargin}{\labelsep}
        }\item #2 \end{list}\par   % Output in quote mode
     \else                                    %   ELSE  center.
       \hbox to\hsize{\hfil\box\@tempboxa\hfil}  
   \fi}


% Define strut macros for skipping spaces above and below text in a
% tabular environment.
\def\abovestrut#1{\rule[0in]{0in}{#1}\ignorespaces}
\def\belowstrut#1{\rule[-#1]{0in}{#1}\ignorespaces}

% Acknowledgments
\long\def\acks#1{\vskip 0.3in\noindent{\large\bf Acknowledgments}\vskip 0.2in
\noindent #1}

% Research Note
\long\def\researchnote#1{\noindent {\LARGE\it Research Note} #1}

\renewcommand{\appendix}{\par
  \setcounter{section}{0}
  \setcounter{subsection}{0}
  \def\thesection{\Alph{section}}
\def\section{\@ifnextchar*{\@startsiction{section}{1}{\z@}{-0.24in}{0.10in}%
             {\large\bf\raggedright}}%
{\@startsiction{section}{1}{\z@}{-0.24in}{0.10in}
             {\large\bf\raggedright Appendix\ }}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               PROOF, THEOREM, and FRIENDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\newtheorem{example}{Example} 
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma} 
\newtheorem{proposition}[theorem]{Proposition} 
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{axiom}[theorem]{Axiom}

==> sections/methods_level2_backup.tex <==
\subsection{Level 2. Data driven compression methods}
\label{section:level_2}
\subsubsection{Per-layer data-optimized SVD methods}

All level 1 compression methods minimize the kernel approximation error. This does not use any information of the actual data which is being processed by the layer of the network. One of the ways to improve level 1 methods is to formulate a method that would rather minimize the error in the activations produced by the compressed layer. A method based on minimizing the error of the output for the specific data allows one to significantly decrease the accuracy loss after the compression. This section describes multiple approaches for per-layer data-optimized SVD compression, as introduced in~(\cite{zhang2016accelerating}). 


\noindent\textbf{Data SVD.} Given an input vector $x \in \mathbb{R}^{k^2s}$, the response $y \in \mathbb{R}^{t}$ is given by

\begin{equation}
\mathbf{y} = \mathbf{W}\mathbf{x}+\mathbf{b}.    
\end{equation}
Assuming that the output data lies on a linear manifold of rank $r$, the optimal projection matrix $\mathbf{M} \in \mathbb{R}^{T\times T}$ is given as a solution of the following optimization problem:

\begin{equation}
\begin{aligned}
& \underset{\mathbf{M}}{\text{argmin}}
& & \norm{\mathbf{Y}-\mathbf{M}\mathbf{Y}}^2_F \\
& \text{s.t.}
& & \rank \mathbf{M} \leq r.
\end{aligned}
\label{eq:data_svd}
\end{equation}
where $\mathbf{Y}\in \mathbb{R}^{t\times n}$ is a matrix which concatenates $n$ responses from the output. We assume the responses have zero mean, for notational simplicity.
The solution is given by principal component analysis (PCA) as follows. Given the eigendecomposition of the covariance matrix $\mathbf{Y}\mathbf{Y}^T=\mathbf{U}\mathbf{S}\mathbf{U}^T$, the value of $\mathbf{M}$ is given by:

\begin{equation}
\mathbf{M}=\mathbf{U}_{r}\mathbf{U}_{r}^T,    
\label{eq:data_svd_low_rank}
\end{equation}
where $\mathbf{U}_{r}$ are the first $r$ are eigenvectors. 
This solution for $\mathbf{M}$ can be used to approximate the original layer. Under the low rank assumption for vector $\mathbf{y}$, the output can be expressed as:

\begin{equation*}
\mathbf{y}=\mathbf{M}\mathbf{W}\mathbf{x} + \mathbf{b}, 
\end{equation*}
where $\mathbf{x}$ is the input vector and $\mathbf{b}$ is the bias. Using (\ref{eq:data_svd_low_rank}), the original kernel can be approximated as $\mathbf{\widetilde{W}}=\mathbf{W_1}\mathbf{W_2}$, where $\mathbf{W}_1=\mathbf{U}_{R}$, and $\mathbf{W}_2=\mathbf{U}_{R}^T\mathbf{W}$. This method corresponds to a data-optimized version of the weight SVD decomposition (\ref{eq:weight_svd}).

\noindent\textbf{Asymmetric data SVD.}
One of the main issues in neural network compression is accumulation of error when compressing a deep model. An asymmetric formulation was introduced in order to alleviate this issue in~\cite{zhang2016accelerating}. As opposed to optimizing the reconstruction error for the approximated layer based on the original input data, the asymmetric formulation is based on the input data from the previous approximated layer. This approach allows one to significantly reduce the full-model accuracy drop in level 2 settings using a limited amount of input data at the cost of solving a more general optimization problem. The following objective is minimized:

\begin{equation}
\begin{aligned}
& \underset{\mathbf{M}}{\text{argmin}}
& & \norm{\mathbf{Y}-\mathbf{M}\mathbf{W}\widehat{\mathbf{x}}}^2_F \\
& \text{s.t.}
& & \rank \mathbf{M} \leq r.
\end{aligned}
\label{eq:opt_gsvd}
\end{equation}

Where $\mathbf{Y}$ is a matrix concatenating the original outputs, $\widehat{\mathbf{x}}$ is an output of the previous approximated layer, and $\widehat{\mathbf{Y}}$ is a matrix concatenating outputs of the compressed layer (columns of $\mathbf{Y}$ and $\widehat{\mathbf{Y}}$ are assumed zero mean for the notation simplicity):

\begin{equation*}
\widehat{\mathbf{y}} = \mathbf{M}\mathbf{W}\widehat{\mathbf{x}}+\mathbf{b}.   
\end{equation*}

The solution is given by the generalized SVD (\cite{takane2006generalized}) on the matrix $\widehat{\mathbf{M}}=\mathbf{Y}\widehat{\mathbf{Y}}^T(\widehat{\mathbf{Y}}\widehat{\mathbf{Y}}^T)^+$ with generalized orthogonality constraints $\mathbf{U}^T\mathbf{U}=\mathbf{I}$ and $\mathbf{V}^T\widehat{\mathbf{Y}}\widehat{\mathbf{Y}}^T\mathbf{V}
=\mathbf{I}$, where $\mathbf{U}$ and $\mathbf{V}$ are given by the following SVD factorization:
\begin{equation}
\widehat{\mathbf{M}}=\mathbf{U}\mathbf{S}\mathbf{V}^T.
\label{eq:asym_decomposition}
\end{equation}
Given the matrices $\mathbf{U}$ and $\mathbf{V}$, the rank reduced solution is expressed as follows:

\begin{equation}
\mathbf{M}=\mathbf{U}\mathbf{S}(\widehat{\mathbf{Y}}\widehat{\mathbf{Y}}^T)^{-\frac{1}{2}}\mathbf{V}^T,
\end{equation}
where $(\widehat{\mathbf{Y}}\widehat{\mathbf{Y}}^T)^{-\frac{1}{2}}$ is a composition of the pseudo-inverse and the matrix square root. 

The reconstruction error of the asymmetric data SVD can be further improved be incorporating the activation function into the formulation:
\begin{equation}
\begin{aligned}
& \underset{\mathbf{M},\mathbf{b}}{\text{argmin}}
& & \norm{f(\mathbf{Y})-f(\mathbf{M}\hat{\mathbf{Y}}+\mathbf{b})}^2_F \\
& \text{s.t.}
& & \rank \mathbf{M} \leq r.
\end{aligned}
\label{eq:asym_nonlin}
\end{equation}

This problem is solved using the following relaxation:

\begin{equation}
\begin{aligned}
& \underset{\mathbf{M},\mathbf{b},\mathbf{Z}}{\text{argmin}}
& & \norm{f(\mathbf{Y})-f(\mathbf{Z})}^2_F + \lambda \norm{\mathbf{Z}-\mathbf{M}\hat{\mathbf{Y}}-\mathbf{b}}^2_F \\
& \text{s.t.}
& & \rank \mathbf{M} \leq r,
\label{eq:asym_nonlin_relaxed}
\end{aligned}
\end{equation}

    Where $\mathbf{Z}$ is an auxiliary variable, and $\lambda$ is a penalty parameter. The second term of the objective is equivalent to~(\ref{eq:opt_gsvd}). The first term can be minimized using SGD for any activation function, or in the case of the ReLU function, it can be solved analytically (\cite{zhang2016accelerating}). Minimization of  (\ref{eq:asym_nonlin_relaxed}) is performed by using alternating minimization. The first sub-problem corresponds to fixing $\mathbf{Z}$ and solving for $\mathbf{M}$, $\mathbf{b}$, and vice versa for the second sub-problem. Increasing values of parameters $\lambda$ are used through the iterations of the method.

\noindent\textbf{Asym3D.}
The authors of ~\cite{zhang2016accelerating} propose to use the formulation~(\ref{eq:opt_gsvd}) to perform double decomposition based on the spatial and the data SVD methods. Given a spatial SVD factors $\mathbf{W}_v$, $\mathbf{W}_h$, the formulation (\ref{eq:opt_gsvd}) can be applied to the second factor:
\begin{equation}
\mathbf{W} = \mathbf{W}_v \mathbf{M} \mathbf{W}_h = \mathbf{W}_v (\mathbf{M}\mathbf{W}_h^{(1)}) \mathbf{W}_h^{(2)} = \mathbf{W}_v \widetilde{\mathbf{W}}_h^{(1)} \widetilde{\mathbf{W}}_h^{(2)},    
\end{equation}

where $\widetilde{\mathbf{W}}_h^{(1)}$ and  $\widetilde{\mathbf{W}}_h^{(2)}$ are rank reduced versions of the filters $\mathbf{W}_h^{(1)}$ and  $\mathbf{W}_h^{(2)}$. The trade-off between accuracy and the computational complexity in this case is determined by two ranks: $r_s$ is the rank of the original spatial SVD decomposition and rank $r_d$ is the rank of the data optimized decomposition applied to the factor $\mathbf{W}_h$. The final decomposed architecture consists of a $k \times 1$ filter with $r_s$ output channels followed by a $1 \times k$ filter with $r_d$ output channels and a $1\times 1$ convolutional layer with $t$ output channels.

\noindent \textbf{Data optimized spatial SVD.}
The per-layer data optimization methods can be combined with different decomposition approaches. The asymmetric data SVD formulation~(\ref{eq:opt_gsvd}) can be used in two ways. The first way, as described in the original paper~(\cite{zhang2016accelerating}), corresponds to using the low-rank projection $\mathbf{M}$ to perform the decomposition (\ref{eq:asym_decomposition}) of the original weights $\mathbf{W}$. The second way is to use the solution $\mathbf{M}$ to obtain data-aware refinement of weights of a spatial decomposition, this approach is described in the following.

If we consider the optimization problem (\ref{eq:opt_gsvd}) without the constraint on the rank:

\begin{equation}
\begin{aligned}
& \underset{\mathbf{M}}{\text{argmin}}
& & \norm{\mathbf{Y}-\mathbf{M}\mathbf{W}\widehat{\mathbf{x}}}^2_F, 
\end{aligned}
\label{eq:opt_gsvd_full_rank}
\end{equation}

the solution for $\mathbf{M}$ can be used to improve the predictions by refining the weights $\mathbf{W}$ based on some input and output data.

Consider a convolutional layer decomposed using the spatial SVD decomposition (\ref{eq:spatial_svd}). Given the original weights $\mathbf{W}$, the layer can be decomposed into two layers:
\begin{equation}
\mathbf{W}=\mathbf{W}_v \mathbf{W}_h.    
\label{eq:gsvd_spatial}
\end{equation}
After substituting~(\ref{eq:gsvd_spatial}) into~(\ref{eq:opt_gsvd_full_rank}), and denoting $\widehat{\mathbf{x}}_v=\mathbf{W}_h\mathbf{\widehat{x}}$:

\begin{equation}
\begin{aligned}
& \underset{\mathbf{M}}{\text{argmin}}
& & \norm{\mathbf{Y}-\mathbf{M}\mathbf{W}_v \widehat{\mathbf{x}}_v}^2_F.
\end{aligned}
\end{equation}
Given the solution $M$, the data optimized version of filters $\mathbf{W}$ then is given by:
\begin{equation}
\widetilde{\mathbf{W}}=\mathbf{M}\mathbf{W}=(\mathbf{M} \mathbf{W}_v) \mathbf{W}_h.    
\end{equation}
In practice, the refined value $\widetilde{\mathbf{W}}_v=\mathbf{M} \mathbf{W}_v$ can be used instead $\mathbf{W}_v$ for the second layer.

\subsubsection{Channel pruning}
Series of methods introduced in the literature is based on pruning channels of a convolutional filter, in particular the method suggested in~\cite{li2016pruning} is based on the weights magnitude. Another pruning method which is optimized for data was introduced in~\cite{he2017channel}. This method uses lasso feature selection to find the set of channel to prune. 

In order to formulate the pruning method as an optimization problem for data, the authors consider applying a kernel $\mathbf{W}\in \mathbb{R}^{t \times s \times k \times k}$ on input volumes $\mathbf{X}\in \mathbb{R}^{n \times s \times k \times k}$ sampled from the feature map of the uncompressed model, where $n$ is the number of samples. The corresponding output volume $\mathbf{Y}$ is a matrix of shape $n \times t$. The original number of channels is reduced to $s^\prime$ ($0 \leq s^\prime \leq s$) in a way that the reconstruction error for the output volume is minimized:

\begin{equation}
\begin{aligned}
& \underset{\beta, \mathbf{W}}{\text{argmin}}
& & \norm{\mathbf{Y}-\sum_{i=1}^{s}\beta_i \mathbf{X}_i \mathbf{W}_i^T}^2_F \\
& \text{s.t.}
& & \norm{\mathbf{\beta}}_0 \leq s',
\end{aligned}
\end{equation}

where $\mathbf{X}_i \in \mathbb{R}^{n \times k \times k}$ is an i-th channel of the input volume and $\mathbf{W}_i \in \mathbb{R}^{N \times k \times k}$ is i-th channel of the filter. Vector $\mathbf{\beta}$ is the coefficient vector for channel selection. If the value $\beta_i=1$ then the corresponding channel can be pruned. In order to solve the problem $L_0$ norm is relaxed to $L_1$ and the minimization is formulated as follows:

\begin{equation}
\begin{aligned}
& \underset{\beta, \mathbf{W}}{\text{argmin}}
& & \norm{\mathbf{Y}-\sum_{i=1}^{s}\beta_i \mathbf{X}_i \mathbf{W}_i^T}^2_F + \lambda \norm{\mathbf{\beta}}_1 \\
& \text{s.t.}
& & \norm{\mathbf{W}_i}_F = 1.
\end{aligned}
\label{eq:channel_pruning}
\end{equation}

The minimization is performed in two steps by fixing $\mathbf{\beta}$ or $\mathbf{W}$ and solving the corresponding sub-problems.
